Baseline functionality for security and control of commodity IoT devices and domain-controlled device lifecycle management

The emerging Internet of Things (IoT) drastically increases the number of connected devices in homes, workplaces and smart city infrastructures. This drives a need for means to not only ensure confidentiality of device-related communications, but for device configuration and management---ensuring that only legitimate devices are granted privileges to a local domain, that only authorized agents have access to the device and data it holds, and that software updates are authentic. The need to support device on-boarding, ongoing device management and control, and secure decommissioning dictates a suite of key management services for both access control to devices, and access by devices to wireless infrastructure and networked resources. We identify this core functionality, and argue for the recognition of efficient and reliable key management support---both within IoT devices, and by a unifying external management platform---as a baseline requirement for an IoT world. We present a framework architecture to facilitate secure, flexible and convenient device management in commodity IoT scenarios, and offer an illustrative set of protocols as a base solution---not to promote specific solution details, but to highlight baseline functionality to help domain owners oversee deployments of large numbers of independent multi-vendor IoT devices.

==> scoping.tex <==
%!TEX root = kmi-for-iot.tex

\section{Scoping Questions (internal notes)}

\newtheorem{question}{Question}
\begin{question}[Need for public keys]
	Are public keys required in the Home environment?
\end{question}
Manufacturer-provided public key certificates provide a means to verify device authenticity (e.g., via remote attestation), if the verifier has a trusted public key to verify the certificate. However, this does not provide a way to establish \emph{trust domains}, i.e., domains of devices belonging to the same owner or managed by the same delegated authority and permitted to communicate with each other.

Also: need device authenticity be verified in all cases?

\begin{question}[Integrity of devices]
	Is device integrity relevant in our setting? How can we detect device tampering or take it into account?
\end{question}
If public key is used, we must consider if HW-based security mechanisms are needed to protect the device private key. Otherwise an adversary may clone devices by extracting a legitimate-device private key and installing it into counterfeit devices.
%
In most cases, we should assume any secret device key is (eventually) leaked.



\begin{question}[Management]
	What management models are possible (centralized, distributed)? Who would take responsibility of centralized management?
\end{question}
Possible options: 
1) centralized management by the device manufacturer, 
2) local management by the trust domain owner (e.g., company; smart home owner), 
3) a hybrid model, trust domain owner delegating device management to an \iotssp{}.  
The business case will determine if the manufacturer has an interest in doing the management. In many cases, they will not want to, or organizational trust domain owners (corporations, government agencies) may not want to externalize management to manufacturers. Thus there needs to be support for distributed management models.

\emph{Handbook Applied Crypto, Ch.13 p.579.
Resurrecting duckling: Ignition keys, Sects. 4.2, 4.3 SW Upload.}

\begin{question}[Delegation]
	Can we support the delegation and re-delegation of device keys to third parties?
\end{question}



\begin{question}[Backups]
	How can keys be backed up, and backups managed? What is persistence model of keys?
\end{question}

If imprinting creates an \emph{ignition key} used to derive authentication and encryption keys, partial recovery from ignition key possible if either key is lost.

But if the ignition key is lost (this will happen sooner or later), it must be replaced by new imprinting, possibly requiring a device ``hard reset". The long-term state of each device should be stored in the \backupservice and restored from there on a re-imprinting.

What must be taken into account to ensure the recovered state is benign, vs.\ a malicious state due to the adversary? In any case, all cryptographic keys used by the device must be re-generated from scratch and not dependent on any information on the device before the point of recovery (possibly known to the adversary).

Should the device be aware that its state has been recovered from backup? For this the \backupservice could maintain metadata (a ``recovery counter") incremented each time the device state is recovered.

\begin{question}[Key updates]
	Is a mechanism for doing key updates on devices (or servers) needed?	
\end{question}

This could limit exposure of encrypted data of past sessions, if key agreement with forward secrecy is used.
Current solutions do not support a convenient mechanism for key updates. Essentially the security association is bootstrapped by registering devices to a cloud user account on first use, where the device is (probably) identified using its public key. \emph{Re-thinking: the device might not actually be authenticated; device registration might be based just on device ID...}

It seems unlikely the keypair is ever updated.

Can a solution employed by OTR (Off-the-Record protocol) \cite{Borisov2004} or Signal (used by WhatsApp) ensure keys are updated? OTR employs numerous DH key agreements, possibly a problem for devices with low computation capabilities. A trade-off between computability and nonrepudiation, forward secrecy might be necessary.

\begin{question}[Persistence]
	How do we take device resets into account, e.g., due to battery replacement? Would device state be lost entirely?
	Can we rely on a reliable counter for resets? How does this relate to SW updates?
\end{question}

If a central \backupservice is present in the local network, it can maintain `version history' metadata about each device. Thus, \localkeymgr can ensure that device firmware is not downgraded (if the device itself does not enforce this). If device state is entirely lost during, e.g., a battery change, it must be re-imprinted and state recovered from the \backupservice.

\begin{question}
	How can we manage device reprovisioning in case a device is resold or reprovisioned?
\end{question}
In current reprovisioning models, users physically do a device `hard reset', wiping out any on-device information. The new owner then must do a new device installation to take ownership---an approach prone to human errors (e.g., failure to reset can leak sensitive information). Asokan and Gene (UC Irvine) are apparently  working in the SeLIoT project~\cite{Seliot2017} on a key management solution based on encrypting the keys on the device using a key that is not permanently stored on the device.

\begin{question}[symmetric/asymmetric key preference]
	Does post-quantum advocate using symmetric keys?
\end{question}

Are asymmetric keys infeasible for low-end sensors? What are the minimal computational requirements?

\begin{question}
	What are root issues for literature attacks? Any taxonomy of errors in IoT device architectures?
\end{question}

Review current attack literature. 
Prominent known attacks (e.g., Mirai) are almost trivial: utilize weak administration passwords or known exploits to access devices.

\begin{question}[Side-channels]
	What is the role of side-channels? What are the possible ways to leak keys?
\end{question}

\begin{question}[Industrial view]
	What are security requirements from corporate viewpoint (CISCO, Intel)?
\end{question}


